Many-Body Coarse-Grained Molecular Dynamics with the Atomic Cluster Expansion

Molecular dynamics (MD) simulations provide detailed insight into atomic-scale mechanisms but are inherently restricted to small spatio-temporal scales. Coarse-grained molecular dynamics (CGMD) techniques allow simulations of much larger systems over extended timescales. In theory, these techniques can be quantitatively accurate, but common practice is to only target qualitatively correct behaviour of coarse-grained models. Recent advances in applying machine learning methodology in this setting are now being applied to create also quantitatively accurate CGMD models. We demonstrate how the Atomic Cluster Expansion parameterization (Drautz, 2019) can be used in this task to construct highly efficient, interpretable and accurate CGMD models. We focus in particular on exploring the role of many-body effects.

==> ace.tex <==
In the remaining of this section, we briefly review how to construct the ACE basis set $B$ and leave the detailed construction to the Appendix~\ref{sec:apd:ACE}. Given relative particle positions $\R_{ji} := \R_j-\R_i$ ($R_{ji}:=|\R_{ji}|$ and $\hat{R}_{ji}:=\R_{ji}/|\R_{ji}|$) and associated chemical elements, one evaluates a one-particle basis
\begin{eqnarray}\label{eq:ace_one}
    \phi_{znlm}(\R_{ji}, z_j) = \delta_{zz_{j}} \mathfrak{R}_n(R_{ji}) \mathfrak{Y}_{lm}(\hat{R}_{ji}),
\end{eqnarray}
followed by a pooling operation resulting in features, 
\begin{eqnarray}
    A_{iznml} = \phi_{znlm}(\R_{ji}, z_j),
\end{eqnarray}
that are denoted the {\it atomic basis} in the context of the ACE model. In \eqref{eq:ace_one} $\mathfrak{R}_n$ are radius basis functions while $\mathfrak{Y}_{lm}$ are spherical harmonic functions. Here we note that the chemical species is not essential in this work since there is no specific chemical species for any CG site, in practice we pick the element that approximately matches the masses of CG sites.

Taking a $\nu$ order (tensor) product results in many-body correlation functions incorporating $\nu+1$ body-order interactions, one can get
\begin{eqnarray}
    {\bf A}_{i\bf znlm} = \prod_{t=1}^{\nu} A_{iz_tn_tm_tl_t}.
\end{eqnarray}
The {\bf A}-basis is a complete basis of permutation invariant functions but does not incorporate rotation or reflection symmetry. An isometry invariant basis {\bf B} is constructed by averaging over rotations and reflections. Representation theory of the orthogonal group $O(3)$ shows that
this can be expressed as a sparse linear operation and results in
\begin{eqnarray}
    {\bf B}_{i} = {\bf C A}_i,
\end{eqnarray}
where $\bth$ contains generalised Clebsch-Gordan coefficients; we refer to~\cite{2019-ship1} for further details.

A major benefit of the linear ACE model is
that the computational cost of evaluating a site energy ${U}^{\rm ACE}_i$ scales only linearly with the number of neighbouring atoms, as well as with the body order $\nu + 1$. This fact reveals the potential efficiency of the ACE-CG model. The question of how to construct ${U}^{\rm ACE}$, as indicated by \eqref{eq:acecg}, is then redirected toward determining the parameter $\bth$, which will be addressed in the following discussion.

